Piecewise Linear Approximation in Data Streaming: Algorithmic Implementations and Experimental Analysis

Piecewise Linear Approximation (PLA) is a well-established tool to reduce the size of the representation of time series by approximating the series by a sequence of line segments while keeping the error introduced by the approximation within some predetermined threshold. With the recent rise of edge computing, PLA algorithms find a complete new set of applications with the emphasis on reducing the volume of streamed data. In this study, we identify two scenarios set in a data-stream processing context: data reduction in sensor transmissions and datacenter storage. In connection to those scenarios, we identify several streaming metrics and propose streaming protocols as algorithmic implementations of several state of the art PLA techniques. In an experimental evaluation, we measure the quality of the reviewed methods and protocols and evaluate their performance against those streaming statistics. All known methods have deficiencies when it comes to handling streaming-like data, e.g. inflation of the input stream, high latency or poor average error. Our experimental results highlight the challenges raised when transferring those classical methods into the stream processing world and present alternative techniques to overcome them and balance the related trade-offs.

==> old/comments.tex <==
%%% INTRODUCTION %%%

% TO DO, read again and let's check we tick all bullets!
\remove{
\begin{tcolorbox}[boxsep=0pt,
                  left=0pt,
                  right=0pt,
                  top=2pt,
                  ]%%
  possible TO DOs when polishing, to connect with the CFP [for ease of ref i copied here "cfp says" (we do)]:
  \begin{itemize}
      \item provide a comprehensive perspective on their strengths and weaknesses, (we see trade-offs)
      
      \item renewed performance evaluation, help to advance the state of the art,(we propose the stream processing perspective and protocols + a method to balance trade-offs)
      
      \item use of open resources (including data or metadata, benchmarks, evaluation tools, or other resources) that benefit the research community or evaluation of research ideas (we use common open sources ...)
      
      \item relevant problems or phenomena and through analysis and/or experimentation provide insights on the nature or characteristics (we propose the scenarios, metrics, ...)
  \end{itemize}
\end{tcolorbox}
}

\remove{ % completely right -> rephrased!
\mpcom{strike through "communication"? they might anticipate something about communication (transmission, etc)  latency}
}


% this is not clear below, any ideas how to improve it ?
% transmitted or stored, to be later (or on reception) reconstructed on-the-fly
% what's the point to process the compress stream on the fly ?? OK, let's remove

\remove{ % exactly!
\mpcom{or processed on-the-fly? (to match the later mention)}
}

% in this situation is irrelevant as firstly it consumes more energy and misses completely the compression objective, and secondly


\remove{ % recent, better ? maybe "recently produced" ? -> OK out!
\mpcom{what is a modern data set?} 
% OK, see tentative comment.
\mpcom{say something first on the first type of results? eg on the trade-off or some other highlight} 
% precis!
\mpcom{the aforementioned?} 
}



\remove{
%%% tentative!!
\romcom{which one is assumed to be relatively small compared to the stream input rate.}
}

%\mpcom{cf the comment on latency, to distinguish from this} --> right, with the addition it makes sense now, I think.



%For instance as it is shown of figure... the 

% VINCENZO NOTES.
% One thing is the technique: angle / linear / convex hull.

% The other thing is the protocols: protocol 1 / protocol 2 / protocol 3

% None of these protocols is actually in the related work, it would be protocol 2 but we are doing something slightly smarter

% Remember that compression can be also expressed in real bytes.

% The paper does not contain a description of the techniques / the 
% protocols are partially there.

% Then there is mixed technique + protocol PLA (which cannot be classified as the others). We got code for this, which could also run angle and convex hull (which would be with protocol 2 simplified).

% There is also that thing about timestamps we have to keep in mind!

% Question: keep in also the last segment?

% Different techniques have been discussed in the literature: angle, linear, convex hull and mixed.
% These techniques differ in the way they approximate the original time series but, in the literature, they all fall short in at least one of the following three things.
% 1) they have been evaluated assuming a batch model (i.e., to compress finite sets of data). That is, the size reduction of a certain technique and the errors introduced in the approximated data have been evaluated using batches of data (usually files) as the base unit. 
% 2) they assumed equally-spaced timestamps (or no timestamps, just sequence numbers)
% 3) not always took the encoding of data into account.

% As we show:
% 1) the quality of each technique applied to generic time-stamped series, is not the same when compressed data is not to be stored but rather transmitted, or when the data source is unbounded (i.e., a stream).
% 2) timestamps can play an important role
% 3) encoding also plays an important role

% We show this and propose 2 variations of the protocol with which data can be stored and transmitted that overcome the limitations of the protocol proposed in the literature.


% or processed on the fly

% \mpcom{maybe name?} 

% \mpcom{we can also call them algorithmic implementations and avoid the term protocols}

% against which we will evaluate PLA streaming  algorithms

%(Some ideas / garbage)
%As we will show in this work, trying to reach the optimal compression given a fixed error might not be what one consider the optimum solution. When trying to minimize the number of output segments, the compression algorithm will tend to get a long compression lines that tend to push the errors toward the threshold. 

%%% PRELIMINARIES %%%

\remove{(see Section~\ref{sec:relatedwork} for works dealing with other versions of the problem)}

%We use the following formalization for the problem of approximating a time series by a piecewise linear representation. 


% are inferior to the aforementioned threshold~$\varepsilon$.
%\mpcom{bf vs emph?}
%NB: here, Vladimir comments may apply but it is not the way PLA has been used so far (see related work) so we just follow the standard way; for unbounded max errors, other techniques are used...

\remove{
that all errors $e_i$ for $i \geq 0$ are inferior to the aforementioned threshold~$\varepsilon$.
}

%\mpcom{show a, b in figures?}
\remove{Figure~\ref{fig:disjointknot} displays a PLA disjoint knot whereas Figure~\ref{fig:jointknot} presents a PLA joint knot}

\remove{
%OK, since we don't use a lot of def, it's more space efficient to rephrase
\mpcom{maybe "manipulated" is not very clear here; process? or some other verb? i am not sure; alternatively, make this a Definitin (as a latex env similar to a lemma) and say that we will need the followind definition in the paper.} }

%%% PLA METHODS %%%

%\subsection{PLA methods}\label{sec:methods}

%(cf Section~\ref{sec:plamedthos} for a description of the main ones found in the recent literature).



\remove{
% first attend of a summary table
\begin{table*}[t!]
    \centering
    \begin{tabular}{c|c|c|c}
        \textbf{PLA method name} & \textbf{Optimization goal} & \textbf{Advantages} & \textbf{Disadvantages} \\
        \hline
        Angle \cite{elmeleegy2009online,xie2014maximum} & Not optimal \mpcom{rephrase?}  & Lowest latency and processing time & Worst compression \\
        Disjoint \cite{elmeleegy2009online,xie2014maximum} & Number of disj. segments & Low latency & $3$ values per segment \\
        Continuous \cite{imai1986optimal,hakimi1991fitting} & Number of cont. segments & $2$ values per segment & Higher number of segments \\
        MixedPLA \cite{luo2015piecewise} & global size & Best compression & High latency \\
        Linear (new) & Balance lat-acc-compr trade-offs(?) & Balancing ... & balancing ...\\
        %\hline \#
    \end{tabular}
    \caption{Summary of the evaluated PLA methods. maybe add complexity? \mpcom{alt: Vladimir's comment about listing good properties and mark entries with v/x ore yes/no/...}}
    \label{tab:plamethods}
\end{table*}
}
% \mpcom{Linear [here]?}


% TABLE (to be inserted here!)
%\mpcom{if it helpw we can think of a table to summarize the key properties of the reviewed methods and techniques}

\remove{
 \mpcom{parts of?}
  \mpcom{i prefer to say "method" than heurstic, but no strong opinion :)}
  % not any more the case
  We shall further develop the two first (historical) approaches, as well as our new method (\S~\ref{linear}), since they will be extended to fit a stream-oriented output framework introduced in Section~\ref{sec:protocols}.
}

\remove{(following the criteria)}
%
% in~\cite{luo2015piecewise} 
% (see each method's description).

%any choice about pursuing the approximation 

% briefly discussed

\remove{ % repeated afterwards
Different methods have been designed with different optimization goals.
% wrong for continuous even though we can qualify it of greedy to
One definitive advantage about a greedy choice lies in the latencies for the reconstruction of the approximated points: since the decision is taken when the segment ends, all points preceding a break-up point can be reconstructed right after the last point of the approximation segment they have been attributed. 
}

%%% removed %%%
%Section~\ref{sec:protocols} is devoted to present this procedure (in \S~\ref{subsec:implicit}) as well as several variants aiming to optimize some performance metrics in our streaming setting.

%A precise definition of the procedure is given in \S~\ref{subsec:implicit}. 


% optimality criteria

%%% removed %%%
%We briefly describe in this section the most cited methods used in the literature, as well as a new heuristic one (\S~\ref{linear}).

%\subsection{Piecewise Constant Approximation}
%For the sake of comparison, we evaluate the performance of the naive piecewise constant approximation. It follows the following naive approach: construct a 

\remove{The first PLA method we consider  is the simplest and oldest one . (which may date from the 70s or earlier, see \S~\ref{sec:relatedwork} for more details)}


\remove{
% repeat I think
An initial angle capturing the zone where next input tuples should be found is
% non-appplicable
in the traditional greedy algorithm,
% obvious
$(x_0,y_0)$ is used as origin and the angle corresponds to the maximum slope line, passing by $(x_1,y_1+\varepsilon)$, and the minimum slope line, passing by $(x_1,y_1-\varepsilon)$.
% repeat
(see Figure~\ref{fig:swingfilter} for an illustration of different cases)
}

%%% removed %%%
%An input point $(x,y)$ modifies the current validity angle as follows (see Figure~\ref{fig:swingfilter} for an illustration of the three cases):
%\begin{itemize}
%\item the error segment associated with $(x,y)$ falls entirely within the angle, both slope lines get updated (point $i$ on Figure~\ref{fig:swingfilter});
%\item the error segment falls at least partially within the angle, one slope line only get updated (point $i+1$ for maximum slope and $i+2$ for minimum slope on Figure~\ref{fig:swingfilter});
%\item the error segment falls entirely outside the angle, then the compression stops (point $i+3$ on Figure~\ref{fig:swingfilter})): no approximation line exist passing through the origin and including all points up to $i+3$. 
%\end{itemize}

\remove{% will be discussed in related work section to save space
This method was recently rediscovered \mpcom{let's quote the paper that mentioned about "rediscovering"; it might be better so} in~\cite{elmeleegy2009online} and presented under the name \textit{SwingFilter}.}



%%% obvious %%%
%It is clear just from the description that the test and update per point uses always constant time. 

%%% related work %%%
%Note, this method was recently rediscovered in~\cite{elmeleegy2009online} and presented under the name \textit{SwingFilter}. 

% ; it corresponds to the 

\remove{
The method is important not only for its simplicity but also for 
%a major advantage relatively to the other ones: 
its guaranteed upper-bound on processing time. 
%Indeed, 
Contrary to all other methods which achieve a constant \textit{amortized} processing time per input tuple, the greedy approximation achieves a \textit{worst-case} $\mathcal{O}(1)$ processing time which can represent an undeniable advantage in some applications. 
}



% this goes to the paragraph to save space and better comprehension
\remove{In the evaluation, the method is named \textit{angle}.}

%\subsection{ConvexHull-based: Longest line segment Approximation}


\remove{ % uselessly complicated
 Recall the \textit{convex hull} of a set of points is the minimum convex set containing all of them and is characterized by its polygonal border in 2 dimensions.
 % repeat
  namely the lower and upper components (Figure~\ref{fig:hull} gives an example)
}

%%% removed %%%
%(considering the $x$-extremal points to be part of both components).


%Let use describe more formally those two partial convex hulls. Let $L_i = \{(t_i,y_i-\varepsilon)\}$ the set of the $i$ first lower endpoints of the error segments, and $U_i = \{(t_i,y_i+\varepsilon)\}$ the one of their upper end points. For definition purpose, we introduce four fictional points passing by two y-lines, namely $m_i = \min_{0 \leq j \leq i} \{y_j -\varepsilon -1\}$ and $M_i = \max_{0 \leq j \leq i} \{y_j +\varepsilon +1\}$. We define the lower convex hull of the $i$ first processed points as the convex hull of the set $L_i \cup \{(x_0,m_i),(t_i,m_i)\}$ and reciprocally the upper lower hull of the same points as the convex hull of the set $U_i \cup \{(x_0,M_i),(t_i,M_i)\}$. We are interesting here in maintaining the continuous segment portions of those two hulls that do not contain fictional points. See Figure~\ref{fig:hulls} for an example of those hulls; the parts we are interested in correctly maintaining are the upper and lower thick lines of the convex hulls. In our context, two specific half-hulls are particularly interesting: the upper part of the lower error endpoints convex hull, that we name \textbf{min hull}, and the corresponding \textbf{max hull} formed by the lower part of the upper error endpoints convex hull. 

\remove{ % let us check what is important here ??
The two partial hulls can be easily updated when a new error segment shows up. If this addition does not lie within the calculated extreme slope lines, the new point is rejected and an approximation segment is calculated\footnote{The method itself again does not enforce how this part is solved but most implementations pick the  ``average'' of the extreme slope lines since this particular line is forced by definition to stable all error segments involved.}. Otherwise, one or both hulls are updated in a similar way as the \textit{angle} of the greedy PLA. In order to maintain the hulls, two extra variables per hull must be kept and updated, namely the contact points of the two extreme slope lines with the hulls. Finally, notice that updating the partial hulls for a single input point might take up to linear time (in the number of points already processed) but each error endpoint is only processed twice: once while (potentially) being added to the hull, and once while being removed from the hull. Hence, the update is performed in amortized constant time per input tuple.
}




\remove{
% THIS SHOULD BE MOVED TO RELATED WORK AS IT DOES NOT HELP HERE
An optimal solution in terms of number of disjoint segments was already found in 1981 \cite{o1981line}. Nevertheless, unaware of this previous work, Elmeleegy \textit{et al} \cite{elmeleegy2009online} presented an alternative method called \textit{SwingFilter} for computing the optimal disjoint PLA. In our evaluation, we use a version 
%faster in processing time, 
that appeared in~\cite{xie2014maximum}, offering slightly better processing performance by reducing the size of the convex hulls. This reduction is achieved by updating the hulls, taking into account current min-max slope lines (\textit{i.e.} including in the hull $b^0_{min}$, $b^0_{max}$, $y_{min}$ and $y_{max}$ on Figure~\ref{fig:hulls}) and not solely the current input tuple (so the computed hulls contain fewer segments: on Figure~\ref{fig:hulls}, we can see the reduction in the lower hull).
}


\remove{
We refer to this method as \textbf{disjoint} in the evaluation.

% This is completely right, SwingFilter is a variation of this method but strictly speaking it gives different results that what we use and call "disjoint" --> I have to refactor that! 
\mpcom{not clear what "this method" refers to; i conclude it must not be the swing (which is the last refereed to in the last paragraph), since swing appears with its own name in the eval. But maybe i misunderstood something }
}

\remove{% related work
This case is solved optimally by Hakimi and Schmeichel~\cite{hakimi1991fitting} in 1991, implemented a variation of the original algorithm~\cite{imai1986optimal} from 1986. 
% too wordy
Instead of taking the error segment corresponding to the break-up point in order to initialize the convex hulls,
the line offering the most possibilities is kept (instead of the ``center line''). The line segment lying between the break-up point and the last point of the previous approximation segment, is then used to initialized the next approximation step.
Furthermore, it is only after a segment line is calculated, that we can trace back the previous intersection point. 
Hence, this method introduces longer latencies than the previous ones: to output the joint knot connecting two consecutive approximation segments, we need to wait at least to have constructed the next segment line coefficients in the approximation.
}


% at least partially
%(\textit{ie} determine the last point approximated by it)

\remove{
In the evaluation, the method is called \textbf{continuous}.
}

% based on dynamic programming


\remove{parameters to be represented}

%%% related work %%%
%In the experimental evaluation, the authors show that this early output scheme works well in practice with a maximum delay of up to 2-4 segments. However in our context, this increase in delay translates into an often intolerable increase in the latency per point, resulting in an average latency often more than doubled what can be achieved by other PLA methods (cf Section~\ref{sec:evaluation}).
% for the output
%Pushing the approximation to the limit generates higher errors.

\remove{
We keep the original \textbf{mixedpla} name for the method in the evaluation.
}

\remove{ % it's interesting but we don't have results on processing time to show that
Remark that smarter check procedures can be designed to eliminate some portions of the hulls during verification. For instance, since each partial hull can be divided into two monotonic sequences (Figure~\ref{fig:hull} plots those components in different shades), one can safely eliminate one of the sequences by checking the highest/lowest point of the hull. However, in regards to the very small size of the hulls in practice, we observed during the experiments that this does not lead to any significant improvement on processing time.
}

% Note that these quantities are easily computed by only maintaining

\remove{ % too obvious
Note that these quantities are easily computed by only maintaining five variables at each iteration: the sums of $x$'s and $y$'s, the sum of $x$'s squared, the sum of $x.y$ products and the number of points $n$ currently approximated by the best-fit line.
% too much
that should process quickly each new input.
}

\remove{
A naive way to verify if this line stables all error segment 
(and hence is a valid approximation line) is to check for every already processed point $(x,y)$ if the best-fit line is within $\varepsilon$ of $(x,y)$.}



%%% old text
% In this situation, for each $i$ the possible lines to consider is reduced to one, namely the best fit, and the problem reduces to whether such a line is valid or not for $i$ points.
% Heuristically optimizing average error
% ideally while keeping the average error $\frac{1}{n} \sum_i |y_i - a \cdot t_i - b|$ (or other measure of fitness) small. 
% Both components can be refined into two possibly empty monotonic sequences: an increasing north west hull, decreasing north east hull, increasing south east hull and a decreasing south west hull. One may note, the lower error endpoints and the upper error endpoints are line separable (existence of a valid line) if and only if their respective convex hulls do not overlap.

\remove{
This PLA method is named \textbf{linear} in this paper.
}

%%% STREAMING PLA %%%

%\vincom{\begin{itemize}
    %\item About the too long section, I think we can safely split to have protocols and metrics as a separate section.
    %\item About the sentence ``In more details, the input of a compression protocol is the stream of PLA records produced by some PLA method and the output is a stream of compression records [...]": since it is a compression protocol shouldn't the input be the original data and the output the compressed one? I understand this is just a matter of terms, but if the protocols has only to do with the way you reconstruct, maybe de-compression protocol is more appropriate? It might also be confusing that, later on, the figures about the different compression protocols include both the compression and decompression part.
    % yes it depends on terms, here protocol is used on top of a PLA method + reconstruction: the full figure is then call streaming-PLA algorithm. I have to read again and clarify everything though
    %\item I am not 100\% sure about the following comment but, when discussing the metrics, are those consistent with the evaluation graphs? All our evaluation is per-point while compression ratio and latency are defined over r (only error over y). Maybe this is OK, but could it be beneficial to state out directly that is actually per-point?
    % OK, I've added a line to try to clarify this point! about latency, it is defined per point because it uses "i" that depends on the point
%\end{itemize}}

%\mpcom{alt. title: Streaming PLA algorithmic implementations?}

%, that serves as an algorithmic implementation of the PLA method

% here, reformulate, input = stream of input values; PLA method is used to produced compression records


% \mpcom{is it clear for the reader what a compression record is? (how is it different from a PLA record?}

\remove{ % no, not with classical!
Hence, any protocol may work with any PLA method. }

\remove{
\mpcom{maybe compression record?} % -> unfortunately, I already used this term for something else
}


%produced by any of the PLA methods 


% because some parts of the PLA record might be available 




%%% removed %%%
%In Section~\ref{sec:protocols}, the implicit protocol and a variant diminishing delays are reviewed as well as three different additional slightly more elaborated protocols. The presented evaluation survey encompasses divers experiments on contemporary traces to gauge the quality of each of these protocols against three performance metrics.

% RD: I just check, even though output is correct looks like is rather uncommon spelling, so I'll "put" output everywhere!

\remove{% completely said twice!
One may note that our definition of the compression ratio gives the same ratio for all points reconstructed through the same compression record;}

%To fit the scope of the streaming-PLA definition, 

%will reach the limiting error with different frequency and the average might differ. 

%%% PROTOCOLS %%%

\mpcom{Shall we use some special way of refering to the  the new protocols, eg {\sc TwoStream} or \emph{SingleStream} , \emph{SingleStream-V}? or \emph{TwoS, SingleS, SIngleSv} or similar? it can be easier to spot them in the evaluation section}

\remove{ % (1) this might be too early (2) this repeats some stuff in Section 5
As an example, let us consider the \textbf{implicit protocol} that fits the definition in a straightforward way. For each PLA record $r$ produced by a particular PLA method, the implicit protocol produces the compression record $r$ (\textit{i.e.}, it is identical to the corresponding PLA record). Thus depending on the type of knot of the considered record, the associated compression record contains either $2$ or $3$ fields. The reconstruction algorithm is the one given in \S~\ref{sec:preliminaries}.

As stated, the implicit protocol would require an additional bit for each record to differentiate between the two types of records while reading the compression record stream. With this additional bit, we can determine the type of the record used and decide how to proceed for the reconstruction of the next line segment. This problem however does not arise in practice, as all but one PLA methods use only one type of knot. The last method uses a trick explained in \S~\ref{subsec:implicit} to circumvent the use of this extra bit.
}

\remove{ % partial solution for now
\mpcom{alt. title: Streaming protocols algorithmic implementations?}
}

%(copy-paste) For instance, we can imagine an output record as a triplet $(a,b,n)$ where $a$ and $b$ are the coefficients of a simple linear model that approximates the $n$ ``next tuples'' of the input sequence, with respectively $a$ being the line slope and $b$ its $y$-intercept. 

% aforementioned

\remove{
\mpcom{next sentence is not very clear}
We  in a  first time the schemes used in the literature, here named \textit{implicit protocol} and its improved variant, and then described three \textit{protocols} focusing on improving different characteristics of the streaming-PLA compression algorithm.
}

%assuming the compression of a 

 %(including potentially the timestamp channel). 
%In the following, we take the following assumption considering timestamps...

% all use datasets where 

% interesting to implement in volvo very high number of channels

% here, justification about the usefullness of timestamps

%\subsubsection{The implicit protocol}

\remove{
% due to repeats
 and more or less implicitly assumed in PLA works
}

%, \mpcom{not clear:  whereas only a single data was sensed at regular interval (recall in this situation, timestamps can be reconstructed at no extra cost)}; 

%\subsubsection{Improved implicit protocol}\label{subsec:improvedimplicit}


%Note but it is not stated in terms of protocol and hence is only applicable to file storage and not streaming. variant output $<-x, y> <y0> <x,y> <-x,y>$ etc

% dramatically -> highly effective; striking: 

\remove{ % too wordy
Hence limiting the number of points that can be approximated by a single line segment has the side effect of increasing the frequency of the output tuples, giving a worst case constant rate feedback even when the compression rate is at maximum.
}

%%% (((say how to plug PLA method

%This mechanism totally or partially annihilate 

% : $3$ floating point numbers and one integer; ``reconstructed''

\remove{% too verbose!
This claim follows intuitively from the lower limit set in order to compress input tuples: for each channel, a value is either not compressed or replaced among at least $3$ other ones by a $4$ values segment. Therefore this scheme has the strong guarantee to have a worst case compression rate of $100\%$. % when any five consecutive tuples can be approximated within the fixed threshold $\varepsilon$.
}

\remove{\mpcom{not very clear},}

%Encoding $n$ in a byte still results in strictly more than $3$ floating-point numbers to be used where disjoint knots need only $3$.

% We present a variant of this scheme in the next section in order to recover its advantages while optimizing the representation of segments.
% if integers are represented with as many bytes as floating point numbers. 

%\def\bmatrix#1{\left\{\matrix{#1}\right\}}

\remove{are two the coefficients of the line passing through it; , and $n$ is a counter indicating the number of values that are compressed within the segment}

%%as in the previous protocol, 
 
 %%% removed %%%
%This last protocol aims to merge the two previous ones and present a compromised approach in terms of advantages and flaws.


	
% floating point values corresponding, byte, 1 byte are used 
% Line segments can hence replace only up to $256$ input values. When
%This third protocol is a variant of the single stream protocol, aiming at correcting its flaws.


%((( say a percentage

% not enough space I think!
% based on Vladimir comment, it's easier to look at the flow chart

%

%\subsection{Protocols and PLA methods}
%Let us examine how the compression rate is reduced by limiting each segment length (in number of tuples) and the worst case possible inflation.


%%% EVALUATION %%%

 \mpcom{names, cf \S\ref{sec:protocols}}
 
 
%\remove{
%RD:  I tried to write a sentence, but I have to say, not really inspired on this...
%\vincom{Based on a comment from Vladimir, maybe it is good to say why all 3 PLA methods instead of just 1 or 2...}}

% REMOVED THE FOLLOWING
%\footnote{Reported GPS-position calculated by recent smartphones make an average from 4.9m on open sky up to 16.8m on city configuration, from a 2015 study from Standford University \cite{van2015worlds}.} 
%\remove{ %RD: I agree with Vladimir's comment
%A big challenge in this domain is to handle data variability: within a single trace, different mode of transportation makes the characteristics of the stream different. A streaming-PLA compression algorithm should ideally adapt to the different situations (eg changes in recording interval, or velocity of the object) without external intervention.
%\vincom{Vladimir asked for an example here. After reading the paragraph, I am actually thinking it is best to remove it, since the word adaptive might mean different things to different reviewers...}
%}
% I remove the following sentence since we have a dedicated section about the datasets
%We use three datasets containing real traces of sensors' transmissions, as well as a dataset regrouping $85$ time series with different characteristics used in previous PLA experimental evaluations. 

% recovered

% to complete

\mpcom{1.last sentence not clear to me :)} \mpcom{best fit for this paragraph here or in section 6.3? in case we need space or avoid repetition; i must read again though}

% that may be hidden in an average value but cannot be balanced in practice.

%\mpcom{regarding the summary table we discussed a bit earlier, could it make sense to simply enhance Table 2 (or similar) with columns corresponding to the evaluation parameters and write brief/distilled "take-home-messages" there? e.g. "higher-inflation" or "balanced trade-off" ... Not sure how efficient this is, just sharingthe thought in case it is worth trying}
%\vincom{The following text represents the graphs we have right now, but we will change it accordingly once we converge.}

%In order to evaluate the presented techniques and protocols, we take into account the following metrics: compression, error and latency as described in \S~\ref{subsec:performance_metrics}. 
%For each value that is delivered by a certain technique and protocol combination, (1) the compression represents the ratio between the bytes needed to represent the compressed point and the bytes actually needed for the uncompressed one, (2) the error is the absolute difference between the original value and the reconstructed one (this error does not exceed the given error threshold), and, finally, the latency is the difference between the cardinality of a value $v$ and the (subsequent) value that triggers the forwarding of the segment to which $v$ belongs.

%In order to evaluate the presented techniques and protocols, we take into account the following metrics: compression, average error and average latency as described in \S~\ref{subsec:performance_metrics}. For each segment that is delivered by a certain technique and protocol combination (be it a single value or multiple consecutive values), (1) the compression represents the ratio between the bytes needed to represent the compressed segment and the bytes actually needed for the uncompressed one, (2) the average error is based on the errors between each uncompressed and reconstructed values, and, finally, (3) the average latency is based on the difference between a tuple time \vincom{not really, is the number} and the time of the tuples that trigger the reception of the former.

%\romcom{For now, it is not the case, isn't it ?}
%For each dataset, all these metrics are aggregated and presented as averages over %\vincom{a certain length, we will see} and for different maximum error values.
%For each specific maximum error value, the graph presents 13 different \vincom{results}, 9 for the combinations of techniques (list) and protocol(list) and 4 for the classic methods.
%\vincom{Explain also which things are shown in each graph, quartiles, averages and so on...}

%%% some additional criteria -- romaric

%In order to calculate the compression ratio, 

%: \textbf{Low}, with a compression ratio over or close to 100\%, \textbf{Medium}, with a compression ratio about 60-80\% of original data and \textbf{High}, with a compression ratio under 40\% of original data.

%The values are also shown in the titles of the subsequent figures.
% \begin{itemize}
%     \item[] \textbf{Low:} with a compression ratio over or close to 100\%
%     \item[] \textbf{Medium:} with a compression ratio about 60-80\% of original data
%     \item[] \textbf{High:} with a compression ratio under 40\% of original data
% \end{itemize}

%%%

%We refer the reader to 


%for a detailed description of the best performing methods and protocols for the given performance metrics.

%, for each of the 13 methods and protocol combinations given in Table \ref{tab:algo}.

%\mpcom{it might be useful to summarize the discussion of the outcome (lessons learned) in a table; of course this will imply some space issue, but there are trade-offs; let's see what we can do}
%\vincom{the paragraphs that follow are a sort of summary already. One option could be to put it in a bullet form, the other to put it in a table with a catchy title for each entry. If the table spans 2 columns the space utulization could probably be the same...}

%We can conclude the following from the different experiments. 
% Mode!

% compression
% \noindent
% \textbf{Two streams protocol never inflates data, Convex Hull method gives best mean compression.}
% Under low compression phase, all ``classical methods'' inflate data at different level on a regular basis with a non-negligible portion of the input points being represented by up to slightly more than twice as many bytes. The two-streams 
% protocol (used in A1, C1 and L1) is the only safe protocol, never showing inflation of data especially noticeable at low compression mode.

% % latency
% \noindent
% \textbf{Single stream variant and Single stream protocols exhibits lowest latency.}
% Among the three protocols, the Single stream variant protocol exhibits the best latency by using a lower limit for compression allowing bursts of uncompressed values to get reconstructed at an earlier stage. The second best protocol is the Single stream one, since it avoids delay involving singletons.

% % error
% \noindent
% \textbf{Two streams, Single stream and Single stream variant protocols produce smaller errors.}
% Our algorithmic implementations, which introduce no error for uncompressible tuples, drag the error per point towards $0$. In all observed experiments, most errors due to the approximation are lower than errors created while processing time series using classical PLA methodologies. 
% %In particular, the average error is at least half of what is achieved with classical PLA methodologies \vincom{(instead of known techniques, maybe know techniques might make reader think about some other technique...)}.
% The PLA method \textit{linear} based on a heuristic best-fit line compression presents significant improvement on individual errors while presenting similar delays compared with the other PLA methods, and a compression ratio fluctuating between the one obtained with the simpler \textit{angle} method and the one computing the longest line segments \textit{convexhull}. 
%\mpcom{mention balances trade-offs?}


%%% end (to integrate)

% \vincom{Do we use the term max error or something else?}
% \romcom{for me it's fine, I used alternatively ``error threshold''}

% \vincom{In which order should we present the results?}
% \romcom{we can analyze each statistics, and show which pair (protocol, algo) seems the best overall}

% \vincom{Not all the graphs are very easy to read, any ideas about how to have them?}
% \romcom{I agree, let's see... Maybe we can play with max error to have closer results, but it'll be hard to find both interesting and plotable thresholds... another idea, I'm not sure it's easy or readable, is to plot the three statistics for one max error side by side so fig 9 (a) will be max for error 0.1, then first "column" compression, second avg error, third latency, that way we can better "compare" methods but a bit less see directly the influence of max error (we have to switch figures), what do you think about that way ? We will have to put scale on auto and to plot it (on the left/right); still the averages are too close to see really the difference, we have to think a bit more how to present the results...}

% \vincom{Should also remember to describe what statistics we present / how the graph looks like.}
% \romcom{OK.}

% \vincom{for the UCR dataset, we can put the graphs in a single row (if space is needed)}
% \romcom{OK.}

% \vincom{for the UCR dataset the error is 5\% (can you confirm, Romaric?) In that case, the average error graph should also be expressed as a percentage rather than as an absolute value.}
% \romcom{5\% is used in two papers, 1 paper deals between 0.5 and 5\% every 0.5\%. I'm computing some stats now, I think to stick ot our setting we can put three threshold one low (lowest 5\% 0.18) one avg (avg 5\% about 0.57) one high (highest 5\% 1.73); 5\% of the "range" is quite arbitrary especially the range can be determined by two outliers and be way larger than the actual stream...}

% \vincom{For lidar I think the three errors are all too small, that's why the graphs look more or less them same}
% \romcom{cf question about readability}



%\subsection{Some ideas / garbage}
%\romcom{old text to me merged or deleted}
%Let us illustrate this compulsory trade-off between quality in terms of the compression rate and quality in terms of the errors committed when reconstructed the individual stream values. Suppose to conserve a high probability to not report a GPS position\footnote{Reported GPS-position calculated by recent smartphones make an average from 4.9m on open sky up to 16.8m on city configuration, from a 2015 study from Standford University \cite{van2015worlds}.} in the wrong street, we want to enforce a maximum tolerated error of about 10m. By using best fit line compression, we can achieve (complete with experimental data)


%%% RELATED WORK %%%

\remove{
\romcom{I will shorten this section, I have to check what was already written before...}
}
%%% NEED TO BE REDUCE %%%

%%%
%\mpcom{this section include background as well, let's remember to make sure to mention it clearly}


% ~\cite{keogh2001online} PLA etc
%In such stressful scenario, ---> Timestamp order
%Elmondy... Ironically, their own work is a rediscovery of a published 1981 paper from O'Rourke as noticed in .

%\vincom{The paper mentioned by Marina contains an exhaustive list of related papers (in case you did not go through it already). To my understanding, many papers are from other areas so I am guessing the use methods rather than proposing new ones. Could still be good to double-check. I trust your judgment, you had a more exhaustive look on this.}

%\vincom{Just a thought, maybe we could start in the related work saying that all the existing method violate (to a certain extent) the conditions we give, which are reasonable in the real-world applications we have. After that, to give a better impression of exhaustive related work, we could present stuff almost in timestamp order, from the 60 to the recent advances discussing how the change / improve / add and in parallel mention how they "miss" our conditions.}


%%% old text, to be merged here I think -- RD %%%
% The problem of finding a PLA of a time series has been recently revisited  \cite{xie2014maximum,luo2015piecewise} while focusing on some of the aforementioned aspects (storage, and time overhead). However, those recent works have only focused on one particular aspect and many previous ones did not explicitly consider it as a compression tool. In fact, none of the previous research dealing with piecewise linear approximation take into account the potential increase due to the approximation when the threshold is too small to compress the input stream. % In particular, all algorithms presented so far induce at least a 150\% representation of the input data in the worst case.

% For instance, in~\cite{luo2015piecewise} the authors claim to minimize the global representation of the stream by minimizing the number of ``parameters'' to represent the stream (to be understood as $\langle x,y \rangle$ tuples or $\langle -x, y_1, y_2 \rangle$ triplets of floating-point numbers). We claim here that this approach does not necessarily minimize the representation of the stream (see the discussion in \S for a example) as our non-optimal framework gives equivalent or lower storage files. This is especially apparent when the prescribed error threshold has been chosen too small to gain anything using linear compression, or the data are not prone to such a compression (highly concentrated within a small zone with, see figure...). 
% In this situation, representing the stream by line segments often induce to remember two values per data point whereas only a single one would have suffice (considering the timestamps are easily compressible or can be omitted, see discussion \S). 


%% HERE -- put every copy-paste into comments %%%

%We have drawn reasonable conditions or requirements for PLA algorithms to be evaluated against realistic data streams. It appears that all existing algorithms focusing mainly on optimizing the number of line segments or another related parameter do not adequately meet our requirements to be efficiently deployed in real-world applications. Such scenarios advocate a better balanced trade-off between precision loss and saved space storage, as well as induced algorithm complexity and reconstruction delay and compression rate. The miss of the target in existing work is, as we shall discuss here, more due to the way existing line construction techniques have been (iteratively) evaluated that the methods themselves.

%% copy paste
% Recall, in order to be valid, an approximation line segment has to intersect every single error segment of the points involved, or otherwise stated has to be a stabbing line for those line segments. 




\remove{ % repeat, useless
As we stated in the introduction, finding a PLA representation of time series is an old problem that has recently found new interests.
}

% We share the point of view already adopted by


\remove{% it's a bit too strong
, and we think their claim has maybe not finished to be implemented. }

%%% remove %%%
%In this section, we shall briefly review the most recent influential works that led to the present work.

\remove{ % too imperative!!
We point the reader to the different references we give in this section for an extensive list of applications of PLA techniques and variants.
}

\remove{
Finding a PLA in order to try to optimize the average error or other related error, new methods have been developed in the literature (eg~\cite{keogh2001online} is a well-known one), but in those cases, the individual maximum error is unbounded.
}


\remove{ 
%% remove from here, where to put, dunno, or at least rephrase... %%%
The other most important parameter of PLA representations concerns the constraint placed on approximation segments jointures. In the general case (also called \text{disjoint} case) two successive segments do not have to share their endpoints, whereas in the \text{continuous} version, every approximation segments must start exactly where the previous one has ended. In our context, forcing a continuous approximation which is more constrained that the disjoint one, has completely lost its original geometrical advantage but keeps a memory-saving superiority since only a single point $(t,y)$ is needed to represent two endpoints. %The continuous case was optimally solved in 1991 \cite{hakimi1991fitting}.

% this repeats what we already say
Most, if not all, known methods to produce PLA representations fall within one of the following three categories and their variants:
\begin{enumerate}
	\item \textbf{angle based techniques} are those where only a constant number of information is kept and evaluated at each processed data: the decision to pursue approximation is a simple check if the new value falls within a cone from some initial point;
	\item \textbf{convex hull techniques} record the convex hulls formed by the error line segments and construct successive longest possible line approximations -- this category finds PLA with least number of segments;
	\item \textbf{dynamic programming techniques} are used to find optimal solutions when the output is not required to be only line segments: those techniques require an additional adaptation to outputs values along the way in order to be used in an online fashion.%, and imply a worst case linear complexity for outputting.
\end{enumerate}
% generally
%  (which can potentially contain all processed points)
%%%
}

\remove{
Early work in PLA focus on approximations of 2D-curves. The general problem considered there is slightly more general as input are not received in increasing $t$-axis order. In particular, ``scan-along implementations'' seek to construct a PLA while turning around the 2D-curve, and with (most often not mentioned) constant amortized time per node. Note however that all algorithms solving such a problem can also be applied to our situation in order to approximate a timestamped stream. Already in 1974, Tomek \cite{tomek1974two} gives a constant-time solution to the case where the curve is a function of a single variable, which happens to be exactly our setting. However, his procedure is purely heuristic and is not optimal. Since then, considerable amount of research has been produced to find optimal PLA (in number of segments) with different error criteria (see e.g. \cite{wu1993new} which gives a brief overview of all techniques). }

\remove{those two algorithms are archetypes of our two first classes, respectively ``angle'' and ``convex hull'' methods}

\remove{Moreover, the paper presents a technique to improve the purely greedy ``angle'' algorithm by using the intersection lines of several points to pick the origin of the angle; they show that increasing the number of initial points used to start the compression procedure leads as intended to better compression (fewer segments) and an increased processing time.}

% what we call here the ``convex hull'' algorithm, a slightly improved version  of the \textit{SlideFilter} procedure
% (regarding processing time)

\remove{
This reduction is achieved by updating the hulls, taking into account current min-max slope lines (\textit{i.e.} including in the hull $b^0_{min}$, $b^0_{max}$, $y_{min}$ and $y_{max}$ on Figure~\ref{fig:hulls}) and not solely the current input tuple (so the computed hulls contain fewer segments: on Figure~\ref{fig:hulls}, we can see the reduction in the lower hull).
}

\remove{needs only to keep track of $5$ instances of the problem to compute the optimal PLA.}

%Luo \textit{et al} remark that minimizing the total number of segments might not effectively minimize the needed space to store the PLA representation. They remark that to encode an approximation by segments two type of nodes can be used: joint node $\langle x,y \rangle$ (when two consecutive approximation segments share an endpoint) or discontinuous node $\langle x,y_1,y_2 \rangle$ (recording a time $x$ between two); a sign trick (storing $-x$ instead of $x$) is used not to have to store an additional bit while streaming output tuples. The article presents a dynamic programming solution scan-along procedure to optimize the ``size'' of the approximation, where for each approximation segment a joint node is counted as $2$ and a disjoint node as $3$ values. 

%We further claim that their measurement is not optimal either as it requires high precision on floating numbers while a different mechanism to output tuples can lead to further space saving (see ...)

% less interesting
%The authors also formally prove that any PLA compression algorithm would need to remember $\Omega(n)$ points (worst case convex hull size) to be correctly able to predict if one error point violate ...

%%% CONCLUSION %%%

%Conclusions... 
% postulate, for data reduction

%This framework is general enough to ease further research and experimental settings with a common criteria for the compression's performance.

%new research: adaptive methods that can switch between protocols to minimize delay and maximize compression.

%out of the scope of the present work but would be interested to set up a complete transmission reduction scenario.

%all introduced methods are relatively
%evaluation of computational overhead in a streaming implementation
%to be able to run efficiently even on small devices

%%% new %%%

The combination of a particular protocol with a particular PLA method will be identified in the rest of the paper as a streaming-PLA algorithm.\mpcom{... and here (cf my comment earlier i this subsection}

\mpcom{doublecheck terms here and ... (end of this subsection)}

% fluctuating nearby the one obtained with the simpler Angle method and the one computing the longest line segments Convex Hull
